Global Control for Local SO(3)-Equivariant Scale-Invariant Vessel Segmentation

Personalized 3D vascular models can aid in a range of diagnostic, prognostic, and treatment-planning tasks relevant to cardiovascular disease management. Deep learning provides a means to obtain such models automatically from image data. Ideally, a user should have control over the included region in the vascular model. Additionally, the model should be watertight and highly accurate. To this end, we propose a combination of a global controller leveraging voxel mask segmentations to provide boundary conditions for vessels of interest to a local, iterative vessel segmentation model. We introduce the preservation of scale- and rotational symmetries in the local segmentation model, leading to generalisation to vessels of unseen sizes and orientations. Combined with the global controller, this enables flexible 3D vascular model building, without additional retraining. We demonstrate the potential of our method on a dataset containing abdominal aortic aneurysms (AAAs). Our method performs on par with a state-of-the-art segmentation model in the segmentation of AAAs, iliac arteries, and renal arteries, while providing a watertight, smooth surface representation. Moreover, we demonstrate that by adapting the global controller, we can easily extend vessel sections in the 3D model.

==> figures/data_benchmark_fig.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\textwidth]{images/data-benchmark-plot.pdf}
    \caption{Data efficiency benchmark.
    We showcase how our method performs based on the number of patients we train it on (for one patient we have 100-200 contours annotated). Results indicate good model performance even when trained on just $3$ patients. \todo[inline]{Combine into 1 figure with DSC for artery ablation}}
    \label{fig:data-efficiency}
\end{figure}
